Off-Policy Evaluation for Action-Dependent Non-Stationary Environments

Methods for sequential decision-making are often built upon a foundational assumption that the underlying decision process is stationary. This limits the application of such methods because real-world problems are often subject to changes due to external factors (passive non-stationarity), changes induced by interactions with the system itself (active non-stationarity), or both (hybrid non-stationarity). In this work, we take the first steps towards the fundamental challenge of on-policy and off-policy evaluation amidst structured changes due to active, passive, or hybrid non-stationarity. Towards this goal, we make a higher-order stationarity assumption such that non-stationarity results in changes over time, but the way changes happen is fixed. We propose, OPEN, an algorithm that uses a double application of counterfactual reasoning and a novel importance-weighted instrument-variable regression to obtain both a lower bias and a lower variance estimate of the structure in the changes of a policy's past performances. Finally, we show promising results on how OPEN can be used to predict future performances for several domains inspired by real-world applications that exhibit non-stationarity.

==> (NeurIPS CR) OPE under Action Dependent Non-stationarity/header.tex <==
% Get better typography
% \usepackage[protrusion=true,expansion=true]{microtype}		

% Small margins
%\usepackage[top=2cm, bottom=2cm, left = 1cm, right = 1cm,columnsep=20pt]{geometry}


% For basic math, align, fonts, etc.
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{dsfont}
% \usepackage[scr=esstix,cal=boondox]{mathalfa} 

\usepackage{courier} % For \texttt{foo} to put foo in Courier (for code / variables)

\usepackage{lipsum} % For dummy text

% for underlining text

\def\mul#1#2{\color{#1}\underline{{\color{black}#2}}\color{black}}
% \usepackage{soul} 
% \newcommand{\myul}[2][black]{\setulcolor{#1}\ul{#2}\setulcolor{black}}

% For images
% \usepackage{graphicx}
% \usepackage{subcaption}
\usepackage[space]{grffile} % For spaces in image names
\usepackage{cancel} % For diagonally striking out equations

% For bibliography
% \usepackage[numbers]{natbib}

% For links (e.g., clicking a reference takes you to the phy)
\usepackage{hyperref}

% For color
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}
\definecolor{dark-red}{rgb}{0.4,0.15,0.15}
\definecolor{dark-blue}{rgb}{0,0,0.7}
\hypersetup{
    colorlinks, linkcolor={dark-blue},
    citecolor={dark-blue}, urlcolor={dark-blue}
}


% Macros
\newcommand{\yash}[1]{\textcolor{blue}{[#1---yash]}}
\newcommand{\imp}[1]{\textcolor{red}{[IMP: #1]}}
\newcommand{\red}[1]{\textcolor{purple}{#1}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}


% \usepackage{algpseudocode}
% \usepackage[noend,linesnumbered,ruled]{algorithm2e}
% \usepackage[vlined,linesnumbered,ruled,algo2e]{algorithm2e}
% \usepackage[vlined,ruled,algo2e]{algorithm2e}

% \usepackage[algo2e]{algorithm2e} 
% \SetKwProg{Fn}{Function}{}{}
% \let\oldnl\nl% Store \nl in \oldnl
% \newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line

% Miscelaneous headers
\usepackage{multicol}
\usepackage{enumitem}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{bm}

% Table of contents
\usepackage{etoc}

\newcommand{\ind}{\perp\!\!\!\!\perp}

% Commands for organizing theorems and proofs

\usepackage{theoremref}
\mathtoolsset{showonlyrefs}

\newtheorem{defn}{Definition}[]
\newtheorem{rem}{Remark}[]
\newtheorem{thm}{Theorem}[]
\newtheorem{claim}{Claim}[]
\newtheorem{lemma}{Lemma}[]
\newtheorem{prop}{Property}[]
\newtheorem{ass}{Assumption}[]
\newtheorem{cor}{Corollary}[]

% For creating sub-groups of Assumptions/Theorems etc.
\newtheorem{reqm}{Requirement}
% \renewcommand\thereqm{A\arabic{reqm}}

\usepackage{thmtools}
\usepackage{thm-restate}

\declaretheorem[name=Theorem]{rtheorem}
\declaretheorem[name=Proposition]{rproposition}
\declaretheorem[name=Assumption]{rassumption}
\declaretheorem[name=Corollary]{rcorollary}
\declaretheorem[name=Lemma]{rlemma}


% Definitions of handy macros can go here
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\pibopt}{\pi_{b^\star}}
\newcommand{\pib}{{\pi_b}}
\newcommand{\pitheta}{{\pi_\btheta}}
\newcommand{\deltheta}{{\frac{\partial}{\partial \btheta}}}
\newcommand{\delthetatwo}{{\frac{\partial^2}{\partial^2 \btheta}}}
\newcommand{\pieval}{{\pi_e}}
\newcommand{\btheta}{{\boldsymbol\theta}}
\newcommand{\data}{{\mathcal{D}}}
\newcommand{\ope}{{\operatorname{OPE}}}
\newcommand{\pe}{{\operatorname{PE}}}
\newcommand{\variance}{{\operatorname{Var}}}
\newcommand{\covariance}{{\operatorname{Cov}}}
\newcommand{\bias}{{\operatorname{Bias}}}
\newcommand{\mse}{{\operatorname{MSE}}}
\newcommand{\loss}{{\mathcal{L}}}
\newcommand{\horizon}{{l}}

% Auto sized brackets
\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\br}[1]{\autobracket*{#1}}

\DeclarePairedDelimiter\autobrackett{[}{]}
\newcommand{\brr}[1]{\autobrackett*{#1}}

\DeclarePairedDelimiter\autobrackettt{\{}{\}}
\newcommand{\brrr}[1]{\autobrackettt*{#1}}
